Dependable Distributed Computing for the International Telecommunication Union Regional Radio Conference RRC06

The International Telecommunication Union (ITU) Regional Radio Conference (RRC06) established in 2006 a new frequency plan for the introduction of digital broadcasting in European, African, Arab, CIS countries and Iran. The preparation of the plan involved complex calculations under short deadline and required dependable and efficient computing capability. The ITU designed and deployed in-situ a dedicated PC farm, in parallel to the European Organization for Nuclear Research (CERN) which provided and supported a system based on the EGEE Grid. The planning cycle at the RRC06 required a periodic execution in the order of 200,000 short jobs, using several hundreds of CPU hours, in a period of less than 12 hours. The nature of the problem required dynamic workload-balancing and low-latency access to the computing resources. We present the strategy and key technical choices that delivered a reliable service to the RRC06.

==> future-plans.tex <==
\section{Future Plans}

Amongst its statutory obligations, the daily processing of space and
terrestrial radio service notices and the planning of limited radio
spectrum and orbit resources for treaty-related conferences are the
most CPU demanding ITU-R activities. The outcome of the RRC06 has been
the GE06 frequency plan and the related agreement.  The provision of
the GE06 agreement have been applicable since 17 of June 2006.  Like
many other agreements, the GE06 agreement contains procedures for the
modification of the plan and procedures for notification of
assignments into the Master International Frequency Register (MIFR),
which contains all the stations actually in use as notified to the
ITU-R. When a Member States proposes to bring into use an assignment
to a broadcasting station contained in the GE06 plan it needs to
notify to the ITU-R, in accordance with the provisions of the Radio
Regulations, the characteristics of this assignments, as specified in
the agreement, for inclusion in the MIFR.  The plan modification
procedure, in case of addition of new assignments/allotments or of
modification of existing ones, comprises the so-called Coordination
examination, where a coordination contour is calculated around the
center of gravity of the proposed modification according to the
procedure outlined in the agreement. MIFR notification ( as well as a
subset of plan modification) requires the so-called Conformity
examination, which requires the determination of test-points and the
comparison for any of those points of the field strength from the
notified assignments and the field strenght from the plan entry, to
verify if the proposed implementation does not cause more interference
than the recorded plan entry. The details of those procedures and
calculations are outside the scope of this paper, the interested
reader may refer to /cite{RRC06FinalActs}.

Both the plan modification procedures and the MIFR notifications
requires the ITU-R to run complex time-consuming calculations, which
the ITU-R has implemented partly adapting software modules developed
by the EBU, partly writing new ones. The running time depends on the
topology of the assignments/allotments notified. A recent submission
involving 187 related assignments in a Single Frequency Network
configuration took about 40 minutes to process.

In addition, some Member States have already expressed the possible
need of re-planning parts or all of the GE06 planned bands, a process
which would imply a similar (smaller scale) approach to the one
adopted at the RRC06.

After the positive experience with the usage of Grid resources at the
RRC06 , the ITU-R in its effort to staying at the forefront of
technologies, in order to be prepared for future events which may
require even more computing capabilities than the RRC06 and to face
present challenges, is interested in keep experimenting with grid
resources and in investigating additional emerging computing paradigm,
like cloud computing /cite{cloud}, where dynamically scalable
resources are provided as a service over the Internet.

For this purpose the ITU-R has planned a pilot project system, to be
performed in close collaboration with CERN and the ITU Information
technology division, which would involve the seamless usage of a local
distributed infrastructure, grid and cloud resources. The system would
allow Member States to submit via an existing ITU web portal
time-consuming calculation requests and, at the back-end, to schedule
and execute jobs trasparently on the integrated infrastructure.

Concerning the local infrastructure at our disposal for this project,
the ITU-R does not dispose anymore of the PC farm available at the
RRC06, but it has bought three Two-Quad-core Xeon 2.33Ghz servers
which can run efficiently eight parallel processes. The distributed
system design has evolved from the push model (where the server
distributes jobs to the clients via UDP/IP protocol) towards the more
efficient pull model (where the clients directly retrieve from the
database the jobs to be run). The implementation still makes use of
Windows Services, but instead of Perl-script based we are now
developing C\# Windows services. Multiple instances of those services
are then installed at the server according to the pattern described in
/cite{MultiInstanceWS} and concurrency is handled using the properties
of the DataSet.  This system, not yet released for external usage, is
already operational inside ITU-R.







